Asteria: Deep Learning-based AST-Encoding for Cross-platform Binary Code Similarity Detection

Binary code similarity detection is a fundamental technique for many security applications such as vulnerability search, patch analysis, and malware detection. There is an increasing need to detect similar code for vulnerability search across architectures with the increase of critical vulnerabilities in IoT devices. The variety of IoT hardware architectures and software platforms requires to capture semantic equivalence of code fragments in the similarity detection. However, existing approaches are insufficient in capturing the semantic similarity. We notice that the abstract syntax tree (AST) of a function contains rich semantic information. Inspired by successful applications of natural language processing technologies in sentence semantic understanding, we propose a deep learning-based AST-encoding method, named ASTERIA, to measure the semantic equivalence of functions in different platforms. Our method leverages the Tree-LSTM network to learn the semantic representation of a function from its AST. Then the similarity detection can be conducted efficiently and accurately by measuring the similarity between two representation vectors. We have implemented an open-source prototype of ASTERIA. The Tree-LSTM model is trained on a dataset with 1,022,616 function pairs and evaluated on a dataset with 95,078 function pairs. Evaluation results show that our method outperforms the AST-based tool Diaphora and the-state-of-art method Gemini by large margins with respect to the binary similarity detection. And our method is several orders of magnitude faster than Diaphora and Gemini for the similarity calculation. In the application of vulnerability search, our tool successfully identified 75 vulnerable functions in 5,979 IoT firmware images.

==> CompilationEvaluation.tex <==
%AST反编译正确性评估
% 实验设置
%我们使用树编辑距离计算源码AST和二进制代码反编译的AST相似度来评估反编译结果。首先我们采用默认编译配置编译openssl 1.0.1 得到不同的架构二进制文件，这样二进制代码都保留了符号信息。对于架构X86，我们取源码中函数A的AST与其对应二进制函数Aarm反编译得到的AST组成 同源对，源码函数A与其他所有二进制函数组成 非同源函数对。 对于源码中xx个函数，我们共得到xx个同源对，xx个非同源对。对于ARM，我们共得到xx个同源对，xx个非同源对。对于PowerPC， xx个同源对，xx个非同源对。对于X64， xx个同源对，xx个非同源对。对于这些AST对，我们计算其相似度并统计。我们在计算的时候只取了AST大小 大于xx 和小于 xx的AST。

We evaluat the results of IDA Pro decompilation by calculating the tree edit distance between source code AST and binary AST obtained from decompilation. 
We use the OpenSSL dataset described in \ref{dataset} and extract all ASTs from dataset with IDA Pro.
Then we extract all ASTs from source code. For each instruction set, we combine the AST of source code function $S_{a}$ with the AST of its binary version function (e.g. $ARM_{a}$) into a homologous pair. And we combine the AST of $S_{a}$ with the ASTs of all non-identical functions in binary.
Then we get 1428 homologous pairs and 2037756 non-homologous pairs for ARM, 1435 homologous pairs and 2057790 non-homologous pairs for X86, 1428 homologous pairs and 2037756 non-homologous pairs for X64, 1429 homologous pairs and 2040612 non-homologous pairs for PowerPC.
We calculate the similarity of homologous pairs and non-homologous pairs and plot the similarity distribution as shown in the Figure~\ref{fig:compilation_distribution}  
The legend \textit{src-x86} means in the homologous AST pairs, one from source code and one from binary of x86 instruction set.
The legend \textit{src-x86(non-homologous)} means in the non-homologous AST pairs, one from source code and one from binary of x86 instruction set.
We can see that the similarities of all non-homologous pairs are less than 70\%.
The reason that similarity of homologous pairs are less than 100\% is that binary functions change due to compilation optimization such as function inline, loop unrolling, if condition reverse and division becoming multiplication.

\begin{figure}
	\includegraphics[scale=0.5]{pics/compilation_distribution_per_all_wid53_k7.pdf}
	\caption{Similarity Distribution for Source and Binary AST Pairs}
	\label{fig:compilation_distribution}
\end{figure} 



% 结果说明
%如图x所示，对于所有的非同源对，有一个明显的界限，小于这个值的都可以认为是非同源。对于

%总结结论
